The Completed SDSS-IV extended Baryon Oscillation Spectroscopic Survey: BAO and RSD measurements from the anisotropic power spectrum of the Quasar sample between redshift 0.8 and 2.2

We measure the clustering of quasars of the final data release (DR16) of eBOSS. The sample contains $343\,708$ quasars between redshifts $0.8\leq z\leq2.2$ over $4699\,\mathrm{deg}^2$. We calculate the Legendre multipoles (0,2,4) of the anisotropic power spectrum and perform a BAO and a Full-Shape (FS) analysis at the effective redshift $z{\rm eff}=1.480$. The errors include systematic errors that amount to 1/3 of the statistical error. The systematic errors comprise a modelling part studied using a blind N-Body mock challenge and observational effects studied with approximate mocks to account for various types of redshift smearing and fibre collisions. For the BAO analysis, we measure the transverse comoving distance $D_{\rm M}(z_{\rm eff})/r_{\rm drag}=30.60\pm{0.90}$ and the Hubble distance $D_{\rm H}(z_{\rm eff})/r_{\rm drag}=13.34\pm{0.60}$. This agrees with the configuration space analysis, and the consensus yields: $D_{\rm M}(z_{\rm eff})/r_{\rm drag}=30.69\pm{0.80}$ and $D_{\rm H}(z_{\rm eff})/r_{\rm drag}=13.26\pm{0.55}$. In the FS analysis, we fit the power spectrum using a model based on Regularised Perturbation Theory, which includes Redshift Space Distortions and the Alcock-Paczynski effect. The results are $D_{\rm M}(z_{\rm eff})/r_{\rm drag}=30.68\pm{0.90}$ and $D_{\rm H}(z_{\rm eff})/r_{\rm drag}=13.52\pm{0.51}$ and we constrain the linear growth rate of structure $f(z_{\rm eff})\sigma_8(z_{\rm eff})=0.476\pm{0.047}$. Our results agree with the configuration space analysis. The consensus analysis of the eBOSS quasar sample yields: $D_{\rm M}(z_{\rm eff})/r_{\rm drag}=30.21\pm{0.79}$, $D_{\rm H}(z_{\rm eff})/r_{\rm drag}=3.23\pm{0.47}$ and $f(z_{\rm eff})\sigma_8(z_{\rm eff})=0.462\pm{0.045}$ and is consistent with a flat $\Lambda {\rm CDM}$ cosmological model using Planck results.

==> intro.tex <==
\section{Introduction}

Understanding the expansion history of the Universe is one of the crucial questions in cosmology. The latest results from the measurements of the angular temperature and polarisation fluctuations in the cosmic microwave background~\citep{Planck18} and the analysis of type Ia supernovae light curves~\citep{Pantheon} highly favors a Universe that can be described in the framework of General Relativity (GR) by a standard cosmological model, $\Lambda$CDM. In this model, the Universe is made of collisionless cold dark matter (CDM), baryons, photons, and neutrinos and of an unknown component, usually called `dark energy' which behaves as a fluid of negative pressure. In the $\Lambda$CDM context, a cosmological constant $\Lambda$ is inserted in the equation of general relativity to take account of the late-time acceleration of the expansion of the Universe.

In the last 15 years, this picture of the Universe has been shown to work remarkably well using the phenomenon of baryon acoustic oscillations (BAO) in the primordial plasma. BAO leave their imprint on the distribution of matter in the Universe as a characteristic separation scale between matter over-densities. This distance is found in the separation of gravitationally collapsed structures such as galaxies~\citep{boss-dr12} and quasars~\citep{DR14-bao} and can be used as a `standard ruler' by large-scale surveys to measure the evolution of the expansion of the Universe at different epochs. 

As the effort to measure the BAO scale to increasingly better precision continues, large-scale surveys have started to provide valuable information on the linear growth rate of structure. This is of significant importance as it is a promising way to test GR~\citep{LinderCahn07}. 

The growth of structure is measured from coherent peculiar velocities that lead to Redshift Space Distortions (RSDs) along the line of sight~\citep{Kaiser87}. These distortions can be related to $f(z)\sigma_8(z)$, where $\sigma_8(z)$ is the normalization of the linear power spectrum on scales of $8\Mpch$ at redshift $z$ and $f$ is the linear growth rate of structure. Anisotropies in the clustering signal may also appear because the assumed cosmology is different from the true cosmology. This is known as the Alcock-Paczynski effect~\citep{AP} and is key to constraining the cosmological expansion history.

In this paper, we present and analyse the power spectrum of the complete quasar sample of the extended Baryon Oscillation Spectroscopic Survey~\citep[eBOSS;][]{ebossoverview} which is part of the SDSS-IV program~\citep{Blanton+2003}. The observations were made at the $2.5\;\mathrm{m}$ Sloan Foundation Telescope~\citep{gunn06} at the Apache Point Observatory (New Mexico, USA) using the two-arm optical spectrograph of BOSS~\citep{bossspectrometer}. This study is part of a coordinated release of the final eBOSS measurements of BAO and RSD in the clustering of luminous red galaxies \citep[LRG ($0.6<z<1.0$);][]{Bautista+20,GilMarin+20}, emission line galaxies \citep[ELG ($0.6<z<1.1$);][]{Raichoor+20,Tamone+20,DeMattia+20}, and quasars \citep[($0.8<z<2.2$);][]{Hou+20,Neveux+20}. At the highest redshifts ($z>2.1$), the coordinated release of final eBOSS measurements includes measurements of BAO in the Lyman-$\alpha$ forest \citep{Dumasdesbourboux+20}. The cosmological interpretation of these results in combination with the final BOSS results and other probes is found in \citet{Eva}.

Due to their high intrinsic luminosity, quasars can be used as tracers of the large scale structure at high redshifts~\citep{Cro09,Myers+07,RossN+09,Shen+09,white12,Karagiannis+14,Eftekharzadeh+15,Laurent+16}. The Data Release 14 of the first two years of eBOSS data~\citep{Ata+18,Hector,Hou+18,Zarrouk+18} demonstrated how well quasars are suited for cosmological clustering analyses and currently provide the most precise clustering information on large scales in the redshift range $0.8<z<2.2$. With the Data Release 16, the number of quasars is more than doubled. We present the measurement of the redshift space power spectrum with the first three even Legendre multipoles. We perform both a standard `BAO-only' analysis where we focus on the BAO features of the power spectrum and a `full-shape' analysis using the TNS model~\citep{TNS10}. The BAO-only analysis allows us to constrain the Hubble distance, $D_{\mathrm{H}}(z)/r_{\rm drag}$, and the transverse comoving distance, $D_{\mathrm{M}}(z)/r_{\rm drag}$. In addition, we also constrain these two quantities together with the linear growth rate of structure, $f(z)\sigma_8(z)$, using the `full-shape' analysis.

The analysis presented in this paper uses the complete five years of the eBOSS sample and is accompanied by several companion papers. The clustering catalogues used in this analysis are described in~\citet{DR16} and specific information relevant to the complete DR16Q quasar catalogue is given in~\citet{DR16Q}. The quasar mock challenge upon which the model of the power spectrum is tested is described in~\citet{Smith+20}. Approximate mocks used for determining the covariance matrix and testing observational systematic effects are described in~\citet{ZhaoC+20}. The analysis of the quasar sample in configuration space is presented in~\citet{Hou+20} and a consensus analysis of the work presented here is common to both articles. Cosmological implications of the measured quasar clustering properties are discussed in~\citet{Eva}.

This paper is structured as follows. In Section~\ref{sec:Data}, we give an overview of the quasar sample, the estimator of the power spectrum and the set of mocks that we used for the estimation of the covariance and the assessment of the systematic errors. In Section~\ref{sec:BAO}, we discuss the measurement of the BAO scales. In Section~\ref{sec:FS}, we present the full shape analysis and describe the systematic errors that affect the measurement. Our final result, and the consensus analysis performed in our companion paper on the 2-point correlation function analysis, are presented in Section~\ref{sec:conclusion}.

